Speech Synthesis and Control Using Differentiable DSP

Modern text-to-speech systems are able to produce natural and high-quality speech, but speech contains factors of variation (e.g. pitch, rhythm, loudness, timbre)\ that text alone cannot contain. In this work we move towards a speech synthesis system that can produce diverse speech renditions of a text by allowing (but not requiring) explicit control over the various factors of variation. We propose a new neural vocoder that offers control of such factors of variation. This is achieved by employing differentiable digital signal processing (DDSP) (previously used only for music rather than speech), which exposes these factors of variation. The results show that the proposed approach can produce natural speech with realistic timbre, and individual factors of variation can be freely controlled.

==> tables/training_time_comparison.tex <==
\begin{table}
	\centering
	\begin{tabular}{cc}
	\toprule
	Model & Training time \\
	\midrule
	WaveNet & 4-5 days (1 GPU) \\
	WaveGlow & 231 hours (9.6 days) (4 GPUs) (\textit{reported}) \\
	Our Model & 2.5 days (1 GPU) \\
	\bottomrule
	\end{tabular}
	\caption{Comparison of model training times. Our model takes much less time and resources than WaveGlow and WaveNet.\VG{[turn this table (including table caption of course) into text to save space]}}
	\label{tab:train_time_comparison}
\end{table}

